Formalizing the Execution Context of Behavior Trees for Runtime Verification of Deliberative Policies

In this paper, we enable automated property verification of deliberative components in robot control architectures. We focus on formalizing the execution context of Behavior Trees (BTs) to provide a scalable, yet formally grounded, methodology to enable runtime verification and prevent unexpected robot behaviors. To this end, we consider a message-passing model that accommodates both synchronous and asynchronous composition of parallel components, in which BTs and other components execute and interact according to the communication patterns commonly adopted in robotic software architectures. We introduce a formal property specification language to encode requirements and build runtime monitors. We performed a set of experiments, both on simulations and on the real robot, demonstrating the feasibility of our approach in a realistic application and its integration in a typical robot software architecture. We also provide an OS-level virtualization environment to reproduce the experiments in the simulated scenario.

==> concl.tex <==
We showed how to formalize the execution context of BTs and
how to obtain runtime monitors from requirements about the mission of
a robot.  We provided experimental evidence that deliberative-level
control based on BTs can be formalized in a natural yet precise way
and that such formalization can be easily embedded in model-based
design workflows~\cite{ColledanchiseTRO17,biggar2020framework}.
Finally, we demonstrated feasibility of our approach
through its implementation in the software toolchain of a real robot
where BTs provide execution policies at the deliberative-level.
%Our future works will include experiments with scenarios
%richer than the one considered here, a full integration with a
%model-based development stack and investigations about coupling
%on-line monitoring with off-line techniques like static analysis and
%model checking.




==> related.tex <==
\textbf{TO DO}

